A Navigation Logic for Recursive Programs with Dynamic Thread Creation

Dynamic Pushdown Networks (DPNs) are a model for multithreaded programs with recursion and dynamic creation of threads. In this paper, we propose a temporal logic called NTL for reasoning about the call- and return- as well as thread creation behaviour of DPNs. Using tree automata techniques, we investigate the model checking problem for the novel logic and show that its complexity is not higher than that of LTL model checking against pushdown systems despite a more expressive logic and a more powerful system model. The same holds true for the satisfiability problem when compared to the satisfiability problem for a related logic for reasoning about the call- and return-behaviour of pushdown systems. Overall, this novel logic offers a promising approach for the verification of recursive programs with dynamic thread creation.

==> math/defs/executiontree.tex <==
Execution tree:
\begin{itemize}
	\item $\mathcal{T} \subseteq \mathbb{N}^*$ prefix-closed
	\item tree with branching degree at most $k$: $\mathcal{T} \subseteq [k]^*$ prefix-closed
	\item Execution trees: trees with branching degree at most $2$ 
	\item Nodes with out-degree $2$ can be of two types: $call$ and $spawn$
	\item Execution trees also have $5$ relations:
	\begin{itemize}
		\item $Loc \subseteq \mathcal{T} \times \mathcal{T}$ relates a node with its left child
		\item $Abs \subseteq \mathcal{T} \times \mathcal{T}$ relates $call$ nodes with return nodes such that it forms a nesting relation on the paths that are obtained when always moving to the left successor
		\item $Caller \subseteq \mathcal{T} \times \mathcal{T}$ relates a node with the first $call$ node encountered when moving up its parents that does not have its return given by the $Abs$ relation on that path
		\item $Spawn \subseteq \mathcal{T} \times \mathcal{T}$ relates a $spawn$ node with its right child
		\item $Spawner \subseteq \mathcal{T} \times \mathcal{T}$ relates a node with the first $spawn$ node encountered when moving up its parents
	\end{itemize}
	\item $Loc$ is total
	\item $Abs$, $Caller$, $Spawn$, $Spawner$ define partial functions, i.e. are right-unique
\end{itemize}

==> math/defs/semantics.tex <==
We now formally define the semantics of \logicname.
It is defined with respect to an execution graph $G=(V, l, (\rightarrow^d)_{d\in\moves})$ and a fixpoint variable assignment $\mathcal{V} \colon \Fixpoints\to 2^{V}$.
Intuitively, $\llbracket \varphi \rrbracket^G_{\mathcal{V}}$ is the set of nodes of $G$ satisfying $\varphi$ when each fixpoint variable $X$ is interpreted to hold at nodes $\mathcal{V}(X)$.
\begin{definition}[Semantics of \logicname]
	Let $\AP$ be a finite set of atomic propositions, $\Fixpoints$ a set of fixpoint variables, $G=(V, l, (\rightarrow^d)_{d\in\moves})$ an execution graph over $\AP$ and $\mathcal{V} \colon \Fixpoints\to 2^{V}$ be a fixpoint variable assignment. The semantics of a \logicname\ formula over $\AP$ and $\Fixpoints$ with respect to $G$ and $\mathcal{V}$ is then defined by
	\begin{align*}
		\llbracket a \rrbracket_\mathcal{V}^G :=&\quad \{x \in V \mid a \in l(x)\}\\
		\llbracket \lnot \varphi \rrbracket_\mathcal{V}^G :=&\quad V \setminus \llbracket \varphi \rrbracket_\mathcal{V}^G \\
		\llbracket \varphi_1 \lor \varphi_2 \rrbracket_\mathcal{V}^G :=&\quad \llbracket \varphi_1 \rrbracket_\mathcal{V}^G \cup \llbracket \varphi_2 \rrbracket_\mathcal{V}^G \\
		\llbracket X \rrbracket_\mathcal{V}^G :=&\quad \mathcal{V}(X) \\
		\llbracket \bigcirc^f \varphi \rrbracket_\mathcal{V}^G :=&\quad \{ x \in V \mid succ_f(x) \text{ is defined and } succ_f(x) \in \llbracket \varphi \rrbracket_\mathcal{V}^G \} \\
		\llbracket \mu X. \varphi \rrbracket_\mathcal{V}^G :=&\quad \bigcap \{ M \subseteq V \mid \llbracket \varphi \rrbracket_{\mathcal{V}[X \mapsto M]}^G \subseteq M \}\\
	\end{align*}
	for $a\in \AP$, $X\in \Fixpoints$ and $f\in \{l,a,-,p,c\}$.
\end{definition}
We also set $\llbracket \varphi \rrbracket_\mathcal{V}:=\{G\in\ExGraphs\mid v_0\in \llbracket \varphi\rrbracket_\mathcal{V}^G\}$.
For closed \logicname\ formulas $\varphi$, the semantics does not depend on the fixpoint variable assignment and we write $\llbracket \varphi \rrbracket$ for $\llbracket \varphi \rrbracket_\mathcal{V}$ for an arbitrary fixpoint variable assignment $\mathcal{V}$.
For an execution graph $G$, we write $G \models \varphi$ for $G \in \llbracket \varphi \rrbracket$.
Finally, for a DPN $\mathcal{M}$, we write $\mathcal{M}\models \varphi$, iff $G \models \varphi$ for all $G\in \llbracket\mathcal{M}\rrbracket$.

In the formal semantics, we can show that $\mu X. \varphi$ indeed characterises a least fixpoint.
We establish the following lemma:
\begin{lemma}
	Let $S = (G,\mathcal{V},X,\varphi)$ where $G=(V, l, (\rightarrow^d)_{d\in\moves}, \curvearrowright)$ is an execution graph, $\mathcal{V}$ is a fixpoint variable assignment, $X$ is a fixpoint variable and $\varphi$ is a \logicname\ formula in positive normal form.
	Then, the function $\alpha_S: 2^V \to 2^V$ with $\alpha_S(M) = \llbracket \varphi \rrbracket^G_{\mathcal{V}[X \mapsto M]}$ is monotone.
\end{lemma}
Using \cref{prop:tarski}, we obtain:
\begin{corollary}\label{cor:fixpoint-characterization}
	Let $S = (G,\mathcal{V},X,\varphi)$ where $G=(V, l, (\rightarrow^d)_{d\in\moves})$ is an execution graph, $\mathcal{V}$ is a fixpoint variable assignment, $X$ is a fixpoint variable and $\varphi$ is a \logicname\ formula in positive normal form.
	Then, $\llbracket \mu X. \varphi \rrbracket_\mathcal{V}^G$ is the least fixpoint of $\alpha_S$.
	%It has an approximant characterisation $\llbracket \mu X. \varphi \rrbracket_\mathcal{V}^G = \bigcup_{\kappa \geq 0} \alpha_S^\kappa(\emptyset)$ where $\alpha_S^0(M) = M$, $\alpha_S^{\kappa + 1}(M) = \alpha_S(\alpha_S^\kappa(M))$ and $\alpha_S^\lambda(M) = \bigcup_{\kappa < \lambda} \alpha_S^\kappa(M)$ for ordinals $\kappa$ and limit ordinals $\lambda$.
\end{corollary}




==> math/defs/successors.tex <==
Let $G = (V, l, (\rightarrow^d)_{d\in\moves}, \curvearrowright)$ be an execution graph. 
We define multiple successor functions $\Succ_l$, $\Succ_a$, $\Succ_-$, $\Succ_p$ and $\Succ_c$ with signature $V \rightsquigarrow V$.
For $x\in V$, the successor functions are given as follows:
\begin{itemize}
	\item The \emph{local successor} $\Succ_l(x)$ of $x$ is the $\intern$-, $\call$- or $\ret$-successor of $x$.
	
	\item The \emph{abstract successor} $\Succ_a(x)$ of $x$ is the node $y\in V$ with $x\curvearrowright y$ or the $\intern$-successor of $x$, if one of those exists, and undefined otherwise.
	
	\item The \emph{caller} $\Succ_-(x)$ of $x$ is the node $y\in V$ having a $\call$-successor $y'$ such that there are $y_0,\dots,y_n\in V$ with $y_0=y'$, $y_n=x$ and $y_{i+1}=\Succ_a(y_i)$ for all $i\in\{0,\dots,n-1\}$. If no such node exists, the caller of $x$ is undefined.
	
	\item The \emph{parent} $\Succ_p(x)$ of $x$ is the node $y\in V$ such that $y$ has a $\spawn$-successor $z$ and there is a path $z=x_0\rightarrow^{d_1}x_1...\rightarrow^{d_n}x_n=x$ with $d_1,...,d_n\in\moves\setminus\{\spawn\}$. If no such node exists, the parent of $x$ is undefined.
	
	\item The \emph{child} $\Succ_c(x)$ of $x$ is the $\spawn$-successor of $x$, if it exists and undefined otherwise.
\end{itemize}

\begin{lemma}\label{lemma:successorcharacterization}
Let $G=(V, l, (\rightarrow^d)_{d\in\moves},\curvearrowright)$ be an execution graph and $x,y\in V$. 
\begin{enumerate}[(i)]
	\item If $y$ is a $\ret$-successor of $x$, then $y=\Succ_a(\Succ_-(x))$.
	\item If $y=\Succ_a(x)$, then $\Succ_-(x)$ is defined iff $\Succ_-(y)$ is defined and in this case $\Succ_-(x)=\Succ_-(y)$.
	\item If $x\rightarrow^\intern y$, $x\rightarrow^\call y$ or $x\curvearrowright y$, then $\Succ_p(x)$ is defined iff $\Succ_p(y)$ is defined and in this case $\Succ_p(x)=\Succ_p(y)$.
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}[(i)]
	\item
	Since $x\rightarrow^{\ret} y$, there is $z\in V$ with $z\curvearrowright y$ and a path $z=x_0\rightarrow^{d_1}x_1\dots\rightarrow^{d_n}x_n=x$ with $d_1,\dots,d_n\in\moves\setminus\{\spawn\}$. Let $c:=|\{i\in\{1,\dots,n\}:d_i=\call\}|$ and $r:=|\{i\in\{1,\dots,n\}:d_i=\ret\}|$. Since $z$ is defined as the node with a minimal path such that $c>r$, we have $c=r+1$. We now show that 
$\Succ_-(x)=z$. This implies in particular that $y=\Succ_a(z)=\Succ_a(\Succ_-(x))$.
	
	If $r=0$, we have $c=1$ and therefore the path is given by $z\rightarrow^{\call} x$ and thus $\Succ_-(x)=z$.
	
	If $r>0$, let $j:=\min\{i\in\{1,\dots,n\}\mid d_i=\call\}$ and $k:=\max\{i\in\{1,\dots,n\}\mid d_i=\ret\}$. Then we have $x_{j-1}\curvearrowright x_k$, since $d_k=\ret$ and $x_{j-1}\rightarrow^{\call}x_j\dots\rightarrow^{d_{k-2}}x_{k-1}$ is a minimal path such that the number of calls $c'$ is greater than the number of returns $r'$. If there is a $i>k$ such that $d_i=\call$, consider the maximal index with this property. Then we have a path $x_{i-1}\rightarrow^{d_i}\dots\rightarrow^{d_n}x_n=x$ with one call and no return, i.e. we have $x_{i-1}\curvearrowright y$ which is a contradiction since $i-1>k-1\geq j\geq 0$. Thus, since $c=c'+1=r'+2=r+1$ we have $d_i=\intern$ for $i\in\{1,\dots,j-1\}\cup\{k+1,...,n\}$. Since further $x_{j-1}\curvearrowright x_k$, $x_0,\dots,x_{j-1},x_k,\dots,x_n$ is a witnessing sequence to see that $\Succ_-(x)=z$.
	
	\item 
	$\Succ_-(x)$ is defined iff there is a node $z\in V$ having a $\call$-successor $z'$ such that there are $z_0,\dots,z_n\in V$ with $z_0=z'$, $z_n=x$ and $z_{i+1}=\Succ_a(z_i)$ for all $i\in\{0,\dots,n-1\}$. Since  $y=\Succ_a(x)$, we can demand equivalently that $z_n=y$, i.e. $\Succ_-(y)$ is defined and in this case $\Succ_-(y)=z=\Succ_-(x)$.
	
		\item 
$\Succ_p(x)$ is defined iff there is a node $z\in V$ having a $\spawn$-successor $z'$ such that there is a path $z'=z_0\rightarrow^{d_1}\dots\rightarrow^{d_n}z_n=x$ with $d_1,\dots d_n\in\moves\setminus\{\spawn\}$. 
If $x\curvearrowright y$, there is a path $x=z_n\rightarrow^{d_{n+1}}\dots\rightarrow^{d_{n+k}}z_{n+k}=x_{n+k}\rightarrow^{\ret} y$ with $d_{n+1},\dots d_{n+k}\in\moves\setminus\{\spawn\}$. In particular, if $x\rightarrow^\intern y$, $x\rightarrow^\call y$ or $x\curvearrowright y$, there is a path $x=z_n\rightarrow^{d_{n+1}}\dots\rightarrow^{d_{n+k}}z_{n+k}=y$ with $d_{n+1},\dots d_{n+k}\in\moves\setminus\{\spawn\}$. Thus,
we can demand equivalently that $z_n=y$, i.e. $\Succ_p(y)$ is defined and in this case $\Succ_p(y)=z=\Succ_p(x)$.
\end{enumerate}
	
\end{proof}

 \begin{figure}
	\centering
	\begin{tikzpicture}
		\node[draw,circle,line width=1pt,label=$v_0$] at (0,0) (n11) {};
		\node[draw,circle,line width=1pt] at (1,0) (n12) {};
		\node[draw,circle,line width=1pt] at (2,0) (n13) {};
		\node[draw,circle,line width=1pt] at (3,0) (n14) {};
		\node[draw,circle,line width=1pt] at (4,0) (n15) {};
		\node[draw,circle,line width=1pt] at (5,0) (n16) {};
		\node[draw,circle,line width=1pt] at (6,0) (n17) {};
		\node[draw,circle,line width=1pt] at (7,0) (n18) {};
		\node[draw,circle,line width=1pt] at (8,0) (n19) {};
		\node[] at (9,0) (dots1) {\dots};
		
		\node[gray!30] at (1,-1.5) (n21) {...};
		
		\node[gray!30] at (6,-1.5) (n31) {...};
		
		\path[draw,->,red,line width=1pt] (n11) to node[midway,above,black]{\footnotesize$\mathit{int}$} (n12);
		\path[draw,->,red,line width=1pt] (n12) to node[midway,above,black]{\footnotesize$\mathit{int}$} (n13);
		\path[draw,->,line width=1pt] (n13) to node[midway,above]{\footnotesize$\mathit{call}$} (n14);
		\path[draw,->,line width=1pt] (n14) to node[midway,above]{\footnotesize$\mathit{call}$} (n15);
		\path[draw,->,line width=1pt] (n15) to node[midway,above]{\footnotesize$\mathit{ret}$} (n16);
		\path[draw,->,red,line width=1pt] (n16) to node[midway,above,black]{\footnotesize$\mathit{int}$} (n17);
		\path[draw,->,red,line width=1pt] (n17) to node[midway,above,black]{\footnotesize$\mathit{int}$} (n18);
		\path[draw,->,line width=1pt] (n18) to node[midway,above]{\footnotesize$\mathit{ret}$} (n19);
		\path[draw,->,red,line width=1pt] (n19) to node[midway,above,black]{\footnotesize$\mathit{int}$} (dots1);
		
		\path[draw,->,gray!30,line width=1pt] (n12) to node[midway,right]{\footnotesize$\mathit{spawn}$} (n21);
		
		\path[draw,->,gray!30,line width=1pt] (n17) to node[midway,right]{\footnotesize$\mathit{spawn}$} (n31);
		
		\path[draw,->,out=230,in=310,NavyBlue,line width=1pt] (n15) to (n14);
		\path[draw,->,out=230,in=310,NavyBlue,line width=1pt] (n16) to (n13);
		\path[draw,->,out=230,in=310,NavyBlue,line width=1pt] (n17) to (n13);
		\path[draw,->,out=230,in=310,NavyBlue,line width=1pt] (n18) to (n13);
		
		\path[draw,->,out=50,in=130,red,line width=1pt] (n13) to (n19);
		%\path[draw,->,out=50,in=130,red,line width=1pt] (n13) to node[midway,above,black]{\footnotesize$\mathit{sum}$} (n19);
		
		\path[draw,->,out=50,in=130,red,line width=1pt] (n14) to (n16);
		%\path[draw,->,out=50,in=130,red,line width=1pt] (n14) to node[midway,above,black]{\footnotesize$\mathit{sum}$} (n16);
		
		
	\end{tikzpicture}
	\caption{Abstract (\textcolor{red}{red}) and caller (\textcolor{NavyBlue}{blue}) successors in parts of the execution graph from \cref{fig:executiongraph}. Irrelevant edges are gray to improve readability.}
	\label{fig:stacksuccessors}
\end{figure}

 \begin{figure}
	\centering
	\begin{tikzpicture}
		\node[draw,circle,line width=1pt,label=$v_0$] at (0,0) (n11) {};
		\node[draw,circle,line width=1pt] at (1,0) (n12) {};
		\node[] at (2,0) (n13) {...};
		
		\node[draw,circle,line width=1pt] at (1,-2) (n21) {};
		\node[draw,circle,line width=1pt] at (2,-2) (n22) {};
		\node[draw,circle,line width=1pt] at (3,-2) (n23) {};
		\node[draw,circle,line width=1pt] at (4,-2) (n24) {};
		\node[] at (5,-2) (dots2) {\dots};
		
		
		\path[draw,->,line width=1pt] (n11) to node[midway,above]{\footnotesize$\mathit{int}$} (n12);
		\path[draw,->,line width=1pt] (n12) to node[midway,above]{\footnotesize$\mathit{int}$} (n13);
		
		\path[draw,->,YellowOrange,line width=1pt] (n12) to node[midway,left,black]{\footnotesize$\mathit{spawn}$} (n21);
		
		\path[draw,->,line width=1pt] (n21) to node[midway,below]{\footnotesize$\mathit{int}$} (n22);
		\path[draw,->,line width=1pt] (n22) to node[midway,below]{\footnotesize$\mathit{call}$} (n23);
		\path[draw,->,line width=1pt] (n23) to node[midway,below]{\footnotesize$\mathit{ret}$} (n24);
		\path[draw,->,line width=1pt] (n24) to node[midway,below]{\footnotesize$\mathit{int}$} (dots2);
		
		\path[draw,->,dashed,out=40,in=140,gray!30,line width=1pt] (n22) to (n24);
		%\path[draw,->,out=40,in=140,gray!30,line width=1pt] (n22) to node[midway,above]{\footnotesize$\mathit{sum}$} (n24);
		
		\path[draw,->,out=45,in=315,ForestGreen,line width=1pt] (n21) to (n12);
		\path[draw,->,out=90,in=315,ForestGreen,line width=1pt] (n22) to (n12);
		\path[draw,->,out=90,in=315,ForestGreen,line width=1pt] (n23) to (n12);
		\path[draw,->,out=90,in=315,ForestGreen,line width=1pt] (n24) to (n12);
	\end{tikzpicture}
	\caption{Parent (\textcolor{ForestGreen}{green}) and child (\textcolor{YellowOrange}{yellow}) successors in parts of the execution graph from \cref{fig:executiongraph}. Irrelevant edges are gray to improve readability.}
	\label{fig:spawnsuccessors}
\end{figure}

\tbd{Describe/reference figures \cref{fig:stacksuccessors} and \cref{fig:spawnsuccessors} in text}

%definition on trees
\begin{comment}
	\tbd{First define these successor types and semantics on graphs, then describe what it translates to in tree semantics?}
	
	Let $(T,r)$ be an execution tree of a DPN. 
	We define multiple successor functions $\Succ_l$, $\Succ_a$, $\Succ_-$, $\Succ_p$ and $\Succ_c$ with signature $T \to T$.
	For $t\in T$, the successor functions are given as follows:
	\begin{itemize}
	\item The \emph{local successor} $\Succ_l(t)$ of $t$ is the $\intern$- or $\call$-child of $t$, if one of those exist. Otherwise there is a node $t'\in T$ with a $\call$-child $t_c$ and a $\ret$-child $t_r$ such that $t$ is a $\{\intern, \ret\}^{*}$ descendant leaf of $t_c$. In this case we set $succ_l(t):=t_r$.
	
	\item The \emph{abstract successor} $\Succ_a(t)$ of $t$ is the $\ret$- or $\intern$-child of $t$, if one of those exist, and undefined otherwise.
	
	\item The \emph{caller} $\Succ_-(t)$ of $t$ is the node $t'\in T$ such that $t'$ has a $\call$-child $t''$ and $t$ is a $\{\intern,\ret\}^{*}$-descendant of $t''$. If no such node exists, the caller of $t$ is undefined.
	
	\item The \emph{parent} $\Succ_p(t)$ of $t$ is the node $t'\in T$ such that $t'$ has a $\spawn$-child $t''$ and $t$ is a $(\moves\setminus\{\spawn\})^{*}$-descendant of $t''$. If no such node exists, the parent of $t$ is undefined.
	
	\item The \emph{child} $\Succ_c(t)$ of $t$ is the $\spawn$-child of $t$, if it exists and undefined otherwise.
	\end{itemize}
\end{comment}

==> math/defs/syntax.tex <==
\begin{definition}[Syntax of \logicname]
	Let $\AP$ be a finite set of atomic propositions and $\Fixpoints$ be a set of fixpoint variables. The syntax of \logicname\ formulas over $\AP$ and $\Fixpoints$ is defined by
	\begin{align*}
		\varphi ::=&\quad a \mid \lnot \varphi \mid \varphi_1 \lor \varphi_2 \mid X \mid \bigcirc^f \varphi \mid \mu X. \varphi
	\end{align*}
	where $a \in AP$, $X\in \Fixpoints$ and $f\in \{l,a,-,p,c\}$ is the successor type.
\end{definition}

A \logicname\ formula $\varphi$ is called \emph{closed}, if every fixpoint variable $X$ is bound in $\varphi$, i.e. it only appears in a a subformula of the form $\mu X.\psi$.
A formula is called \emph{well-formed}, if every fixpoint variable $X$ (i) is bound by only one fixpoint formula which we then denote by $\fp(X)$, (ii)  appears in the scope of an even number of negations inside $\fp(X)$ and (iii) is in scope of at least one next operator inside $\fp(X)$.
We use $\Sub(\varphi)$ for the set of subformulae of a formula $\varphi$.
The size $|\varphi|$ of a formula $\varphi$ is defined as the number of its distinct subformulae.
We also need a notion of substitution: $\varphi[X:\varphi']$ is the formula that is obtained from $\varphi$ by replcaing every occurrence of the fixpoint variable $X$ with $\varphi'$.

Before introducing further definitions, let us explain the intuition behind each construct.
Atomic formulae $a$ for $a \in \AP$ express that $a$ holds in the current node of the graph.
Next operators $\bigcirc^f \varphi$ can be used to navigate in the graph and express that the $f$-successor exists in the current node of the graph and additionally satisfies $\varphi$.
Negation and disjunction are interpreted as usual.
Finally, we have fixpoint variables $X$ and least fixpoint operators $\mu X. \varphi$ that can be used to specify more involved properties.
Intuitively, $\mu X. \varphi$ is the least fixpoint of a function that repeatedly \textit{unrolls} $\varphi$ by replacing $\varphi$ with $\varphi[X:\varphi]$.
The semantics of $\mu X. \varphi$ is then equivalent to the smallest such unrolling in a given node of the graph.

We use some common syntactic sugar such as $\true \equiv a \lor \lnot a$, $\false \equiv \lnot \true$, $\varphi_1\land \varphi_2\equiv\lnot(\lnot \varphi_1\lor \lnot \varphi_2)$, $\varphi_1 \rightarrow \varphi_2 \equiv \lnot \varphi_1 \lor \varphi_2$, $\varphi_1 \leftrightarrow \varphi_2 \equiv (\varphi_1 \rightarrow \varphi_2) \land (\varphi_2 \rightarrow \varphi_1)$ and $\nu X.\varphi\equiv \lnot \mu X.\lnot \varphi[\lnot X/X]$. 
We also introduce a dual operator $\bigcirc^{\overline{f}}\varphi\equiv \lnot \bigcirc^f\lnot \varphi$ of $\bigcirc^f \varphi$ for $f\in \{a,-,p,c\}$. 
This deals with the problem that $\lnot\bigcirc^f\varphi$ is not equivalent to $\bigcirc^f \lnot\varphi$ for $f\in \{a,-,p,c\}$ since the successor can be undefined for certain nodes in an execution graph.
We also introduce some vairiants of LTL modalities as derived operators.
In particular we use $\varphi_1 \mathcal{U}^f \varphi_2 \equiv \mu X. (\varphi_2 \lor (\varphi_1 \land \bigcirc^f X))$, $\mathcal{F}^f \varphi \equiv \true \mathcal{U}^f \varphi$ and $\mathcal{G}^f \varphi \equiv \lnot \mathcal{F}^f \lnot \varphi$ for $f \in \{l,a,-,p,c\}$.
For $f = l$, we sometimes omit the superscript and write $\mathcal{F} \varphi$ etc.
Intuitively, these modalities correspond to the usual LTL modalities evaulated on the path starting in the current position and taking $f$-successors.
Additionally, we introduce modalities $\mathcal{G}^g \varphi \equiv \nu X. (\varphi \land \bigcirc^l X \land \bigcirc^{\bar{c}} X)$ and $\mathcal{F}^g \varphi \equiv \nu X. (\varphi \lor \bigcirc^l X \lor \bigcirc^c X)$ to express that $\varphi$ holds in all positions or some position, respectively, reachable from the current position.
Using these abbreviations, dual operators and the equivalence $\lnot \lnot \varphi\equiv \varphi$ we can transform every well-formed formula into an equivalent formula in which negation only appears in front of atomic propositions.
We call this form \emph{positive normal form} and assume formulae to be given in this form in the algorithms presented in this paper.

When a formula $\varphi$ is in positive normal form, we use $\ad(\varphi)$ for the fixpoint alternation depth of $\varphi$.
It is a well-established measure for the complexity of nested fixpoint formulae and often, as in our case, a measure for the complexity of algorithmic constructions for fixpoint formulae.
Formally, it is defined as follows.
In a formula $\varphi$, we say that fixpoint variable $X'$ depends of the variable $X$, written $X \prec_\varphi X'$, if $X$ is a free variable in $\fp(X')$.
We write $<_\varphi$ for the transitive closure of $\prec_\varphi$.
Then, the alternation depth $\ad(\varphi)$ is defined as the length of the longest chain $X_1 <_\varphi \dots <_\varphi X_n$ such that adjacent variables have a different fixpoint type, i.e. $\fp(X_i) = \mu X_i . \varphi_i$ and $\fp(X_{i+1}) = \nu X_{i+1}. \varphi_{i+1}$ or vice versa.
For example, if $\varphi(X_1,\dots,X_n)$ is an arbitrary formula in which $X_1,\dots,X_n$ occur freely, then $\mu X. ((\nu X'. \varphi(X')) \lor \varphi(X))$ has fixpoint alternation depth $1$ and $\mu X. \nu X'. \mu X''. \varphi(X,X',X'')$ has fixpoint alternation depth $3$.

==> math/proofs/sat-equivalence.tex <==
\begin{proof}[\textbf{Proof of \cref{thm:satequivalence}}]
	For the first direction, assume that a formula $\varphi$ is satisfiable by a DPN $\mathcal{M}$.
	Then $G \models \varphi$ for all $G \in \llbracket \mathcal{M} \rrbracket$.
	Since $\llbracket \mathcal{M} \rrbracket \neq \emptyset$ (this indeed holds for all DPNs), we can thus choose an arbitrary graph $G \in \llbracket \mathcal{M} \rrbracket$ to show that $\varphi$ is satisfiable by a graph.
	
	For the other direction, assume that a formula $\varphi$ is satisfiable by a graph $G$.
	By \cref{cor:formulatoautomaton}, we know that $\mathcal{T}(G) \in \mathcal{L}(\mathcal{A}_\varphi)$.
	Since $\mathcal{L}(\mathcal{A}_\varphi)$ is a nonempty $\omega$-regular tree language, we know that $\mathcal{T} \in \mathcal{L}(\mathcal{A}_{\varphi})$ for a regular tree $\mathcal{T} = (T,r)$, i.e. a tree with only finitely many non-isomorphic subtrees (see e.g. Cor 8.20. in \cite{Graedel2002}).
	Let $x_1,\dots,x_n$ be the finitely many classes of distinct subtrees of $T$ such that $x_1$ is the class of the root of $T$ and let $r(x_i) = (l_i,d_i,p_i)$ be the label of nodes from class $x_i$.
	We construct a DPN $\mathcal{M} = (\{s\},s,x_1,\Delta,L)$ with stack alphabet $\Gamma = \{x_1,\dots,x_n\}$.
	The labeling $L$ is defined such that $L(s,x_i) = l_i$.
	Transition rules are defined from the parent-child relationships between the different nodes:
	\begin{itemize}
		\item if $d_i = \intern$, then $x_i$ has exactly one child $x_j$ and we include $s x_i \rightarrow s x_j \in \Delta$,
		\item if $d_i = \spawn$, then $x_i$ has exactly one left child $x_j$ and one right child $x_k$ and we include $s x_i \rightarrow s x_j \triangleright s x_k \in \Delta$,
		\item if $d_i = \callret$, then $x_i$ has exactly one left child $x_j$ and one right child $x_k$ and we include $s x_i \rightarrow s x_j x_k \in \Delta$,
		\item if $d_i = \call$, then $x_i$ has exactly one child $x_j$ and we include $s x_i \rightarrow s x_j x_i \in \Delta$,
		\item if $d_i = \ret$, then $x_i$ has no children and we include $s x_i \rightarrow s \in \Delta$ and
		\item if $d_i = \labelend$, then $x_i$ has no children and we do not include a transition for $s x_i$.
	\end{itemize}
	We show that $\llbracket \mathcal{M} \rrbracket = \{ G_0 \}$ where $\mathcal{T} = \mathcal{T}(G_0)$ and thus $\mathcal{M} \models \varphi$.
	It is easy to see that $\llbracket \mathcal{M} \rrbracket$ is a singleton set since $\mathcal{M}$ is deterministic.
	It remains to show that $\mathcal{T} = \mathcal{T}(G_0)$.
	For this, let $\mathcal{T}(G_0) = (T_G,r_G)$.
	
	We show by induction on the length of $x$ that for all $x \in \{0,1\}^*$, $x \in T$ iff $x \in T_G$ and in that case (a) $r(x) = r_G(x)$ and (b) if $x$ has the class $x_i$, then the configuration in $\delta_G^{-1}(x)$ is $(s,x_i w)$ for some stack content $w$.
	In the base case, we know that $\varepsilon \in T$ and $\varepsilon \in T_G$.
	We know that $r(\varepsilon) = (l_1,d_1,p_1)$ since $T$ is rooted in $x_1$ and $p_1 = \bot$ since $\mathcal{T}$ is an execution tree.
	Let $r_G(\varepsilon) = (l,d,p)$.
	Since $(s, x_1 \bot)$ is the starting configuration of $\mathcal{M}$, we know that it is also the configuration in $\delta_G^{-1}(\varepsilon)$ and that $l = l_1$.
	Additionally, we can show that $d = d_1$ by a case distinction on $d_1$.
	We only sketch the case $d_1 = \intern$, the other cases are similar.
	In this case, the only enabled transition in $(s, x_1 \bot)$ is $s x_1 \rightarrow s x_j$, an internal transition.
	Thus, $\delta_G^{-1}(\varepsilon)$ has exactly one $\intern$-successor in $G_0$ which means that $d = \intern$.
	Finally, since $\mathcal{T}(G_0)$ is an execution tree, we have $p = \bot$. 
	
	In the inductive step, we consider $x \cdot d$ for $d \in \{0,1\}$.
	From the induction hypothesis, we know that the claim holds for $x$.
	If $x \not\in T$ and $x \not\in T_G$, then also $x \cdot d \not\in T$ and $x \cdot d \not\in T_G$ since trees are prefix-closed.
	In the other case, let $x_i$ be the class of $x$.
	We have $x \in T$ and $x \in T_G$ with $r(x) = r_G(x) = (l_i,d_i,p_i)$ and the configuration in $\delta_G^{-1}(x)$ is $(s,x_i w)$ for some stack content $w$.
	We distinguish cases based on $d_i$.
	We consider the case where $d_i = \callret$, the other cases are similar.
	Since $\mathcal{T}$ is an execution tree, we know that $x \cdot d \in T$ for $d \in \{0,1\}$.
	Let $x_j$ be the class of $x \cdot 0$ and $x_k$ be the class of $x \cdot 1$.
	We know that the only enabled transition in $(s,x_i w)$ is $s x_i \rightarrow s x_j x_k$.
	Since $d_i = \callret$ and since $\mathcal{T}(G)$ is an execution tree, we know that $\delta_G^{-1}(x \cdot 0)$ continues with the configuration after this call transition and $\delta_G^{-1}(x \cdot 1)$ continues with the configuration after the matching return transition (which exists in this case).
	Thus, the configuration in $\delta_G^{-1}(x \cdot 0)$ is $(s,x_j x_k w)$ and the configuration in $\delta_G^{-1}(x \cdot 1)$ is $(s, x_k w)$, establishing this part of the claim.
	We now establish that $r(x \cdot d) = r_G(x \cdot d)$.
	For the first and second component, this is established by the fact that the configuration in $\delta_G^{-1}(x \cdot d)$ determines both the label and the unique enabled transition.
	For the third component, this follows from the fact that both $\mathcal{T}$ and $\mathcal{T}(G)$ are execution trees and the fact that $r(x)$ and $r_G(x)$ match in the second component.
\end{proof}

==> sections/main/fixpointalternation.tex <==
In this appendix, we define the notion of fixpoint alternation depth for formulae in positive normal form.
%When a formula $\varphi$ is in positive normal form, we use $\ad(\varphi)$ for the fixpoint alternation depth of $\varphi$.
The fixpoint alternation depth is a well-established measure for the complexity of nested fixpoint formulae and often, as in our case, a measure for the complexity of algorithmic constructions for fixpoint formulae.
Formally, $\ad(\varphi)$, the fixpoint alternation depth of a formula $\varphi$ in positive normal form, is defined as follows.
We say that a fixpoint variable $X'$ depends on the variable $X$ in $\varphi$, written $X \prec_\varphi X'$, if $X$ is a free variable in $\fp(X')$.
We write $<_\varphi$ for the transitive closure of $\prec_\varphi$.
Then, the alternation depth $\ad(\varphi)$ is defined as the length of the longest chain $X_1 <_\varphi \dots <_\varphi X_n$ such that adjacent variables have a different fixpoint type, i.e. $\fp(X_i) = \mu X_i . \varphi_i$ and $\fp(X_{i+1}) = \nu X_{i+1}. \varphi_{i+1}$ or vice versa.
For example, if $\varphi(X_1,\dots,X_n)$ is an arbitrary formula in which $X_1,\dots,X_n$ occur freely, then $\mu X. ((\nu X'. \varphi(X')) \lor \varphi(X))$ has fixpoint alternation depth $1$ and $\mu X. \nu X'. \mu X''. \varphi(X,X',X'')$ has fixpoint alternation depth $3$.

==> sections/main/lock.tex <==
\section{Dynamic Pushdown Networks with Nested Locking}

\tbd{Introduce DPN model with arbitrarily many locks (but a fixed number of procedure-local lock variables) from Sebastian's PhD thesis}
\tbd{Show that we can construct a Tree Automaton recognising the execution trees generated from such executions}
\tbd{Size should be something like $|\mathcal{M}|^l$ where $l$ is the number of lock variables}
\tbd{This would enable MC in $\EXPTIME$ for a more powerful model}
